DIFFQG: Generating Questions to Summarize Factual Changes

Identifying the difference between two versions of the same article is useful to update knowledge bases and to understand how articles evolve. Paired texts occur naturally in diverse situations: reporters write similar news stories and maintainers of authoritative websites must keep their information up to date. We propose representing factual changes between paired documents as question-answer pairs, where the answer to the same question differs between two versions. We find that question-answer pairs can flexibly and concisely capture the updated contents. Provided with paired documents, annotators identify questions that are answered by one passage but answered differently or cannot be answered by the other. We release DIFFQG which consists of 759 QA pairs and 1153 examples of paired passages with no factual change. These questions are intended to be both unambiguous and information-seeking and involve complex edits, pushing beyond the capabilities of current question generation and factual change detection systems. Our dataset summarizes the changes between two versions of the document as questions and answers, studying automatic update summarization in a novel way.

==> tab/blrt.tex <==
\begin{table}[h]
\begin{center}
\scalebox{0.89}{
\begin{tabular}{ll|cc}
\toprule
Diff & QG & All & Edited Questions \\
\midrule
Overlapping Answer & Squad &  72.3 & 43.6\\
Q-Dedup & Squad & 72.7 & 50.8 \\
\multicolumn{2}{l|}{Ft on Q-Dedup} & 72.3 & 45.9 \\
\multicolumn{2}{l|}{Ft on Vitamin-C} & 71.1 & 39.9\\
\bottomrule
\end{tabular}
}
\caption{Bleurt scores for all \dataset{} examples and edited question subset.}
\label{tab:blrt}
\end{center}
\end{table}

% Span in Base & Squad-base & 42.6 & 46.4 & -0.29 & 38.7\\
% Q-Dedup & Squad-base & 48.5 & 52.6 & -0.35 & 41.3 \\
% Q-sim & Squad & 47.4 & 51.4 & 51.6 & 55.6 \\

==> tab/edited_questions.tex <==
\begin{table}[ht!]
\begin{center}
\scalebox{0.89}{
\begin{tabular}{lcccc}
\toprule
Model & R-1 & R-L & QSim & BLRT\\
\midrule
SQuAD-same & 42.6 & 46.4 & 38.7 & 45.4 \\ 
SQuAD-sampled & 38.2 & 41.6 & 39.7 & 43.6 \\
SQuAD-reseeded & 37.6 & 40.6 & 41.5 & 43.6 \\
NQ & 14.8 & 28.6 & 18.2 & 29.1 \\
\bottomrule
\end{tabular}
}
\caption{Variance of question generation models on \dataset{} edited questions. We report three different versions of the SQuAD model, where the first model is the same as we used to seed the questions. For factual change detection, we use the heuristic of the overlapping answer. R-1=ROUGE-1, R-L=ROUGE-L, QSim=Query Similarity model-based accuracy, BLRT=BLEURT.}
\label{tab:qg_edited}
\end{center}
\end{table}

==> tab/main_results_w_ques_level.tex <==
\begin{table*}[ht!]
\begin{center}

\begin{tabular}{ll|ccc|ccc|ccc}
% \toprule
\multicolumn{2}{c|}{Models} & \multicolumn{3}{c|}{Diff Detection} & \multicolumn{3}{c|}{Question Level} & \multicolumn{3}{c}{System Level} \\
\midrule
% \cmidrule(lr){1-2} \cmidrule(lr){3-5} \cmidrule(lr){6-8} \cmidrule(lr){9-11}
Diff & QG & P & R & F1 & R-1 & R-L & Qsim & R-1 & R-L & Qsim \\
\midrule
\emph{Pipelined systems} & \\
Overlapping Ans & SQuaD & 79.1 & 74.6 & 76.7 & 60.0 & 63.8 & 65.7 & 70.2 & 71.3 & 71.9 \\
% Ans Equivalence & SQuaD & 84.5 & 64.2 & 73.0 & 74.6 & 77.9 & 69.8 & 74.6 & 75.5 & 73.4 \\
% Qsim & Squad-base & 62.0 & 91.0 & 74.0 & 73.3 & 76.4 & - & 64.6 & 65.7 & - \\
% Span in Base & Squad-base & 79.1% & 74.6% & 76.7% & 62.3% & 66.1% & 65.7% & 70.9% & 72.0% & 71.9% \\
% Q-Dedup & Squad-base & 77.2 & 84.5 & 81 & 73.7 & 76.9 & - & 75.1 & 76.2 & - \\
Q-sim & SQuaD & 65.4 & 93.3 & 76.9 & 58.9 & 62.7 & 63.6 & 62.5 & 63.9 & 64.2 \\
Q-Dedup & SQuaD & 76.7 & 85.5 & 80.9 & 59.4 & 63.0 & 63.9 & 70.2 & 71.4 & 71.7 \\
\midrule
\emph{Joint systems} & \\
\multicolumn{2}{l|}{Ft on Q-Dedup} & 78.4 & 77.1 & 77.7 & 60.1 & 63.1 & 62.1 & 70.3 & 71.2 & 70.9 \\
\multicolumn{2}{l|}{Ft on Vitamin-C} & 79.9 & 71.4 & 75.4 & 55.5 & 58.8	& 52.4 & 68.9 & 69.9 & 68.0 \\
\bottomrule
\end{tabular}

\caption{Full system performance of the pipelined and joint systems on DiffQG. R-1=Rouge1, R-L=Rouge-L, Qsim=Query similarity model based accuracy, Ft=finetuned, Q-Dedup=Query Deduplication}
\label{tab:overall}

\end{center}
\end{table*}

==> tab/qgen_all.tex <==
\begin{table*}[ht]
\begin{center}
\begin{tabular}{l|cccc|cccc}
\toprule
& \multicolumn{4}{c|}{Positive} & \multicolumn{4}{c}{Human Written}
\midrule
Model & R-1 & R-L & QSim & BLRT &  & R-1 & R-L & QSim & BLRT\\
\midrule
SQuAD-seed & 71.7 & 74.9 & 66.3 & 74.1 & 56.5 & 61.4 & 48.2 & 61.3\\
SQuAD-sampled & 59.6 & 63.2 & 57.8 & 65.6  & 50.9 & 55.2 & 47.0 & 58.3\\
SQuAD-retrained & 58.0 & 61.7 & 58.9 & 65.6 & 50.3 & 54.5 & 50.4 & 59.4 \\
NQ & 20.4 & 39.6 & 22.9 & 41.5  & 20.4 & 39.1 & 20.0 & 40.2 \\
\bottomrule
\end{tabular}
\caption{Variation in performance of question generation models on the positive subset of \dataset{}. We report three different versions of the SQuAD model, where the first model is the same as we used to seed the annotations. R-1=ROUGE-1, R-L=ROUGE-L, QSim=Query Similarity model-based accuracy, BLRT=BLEURT.}
\label{tab:qg_all}
\end{center}
\end{table*}
